Searching for magnetic fields in featureless white dwarfs with the DIPOL-UF polarimeter at the Nordic Optical Telescope

About 20% of the white dwarfs possess a magnetic field that may be detected by the splitting and/or polarization of their spectral lines. As they cool, the effective temperatures of the white dwarfs becomes so low that no spectral lines can be seen in the visible wavelength range. If their atmospheres are not polluted by the debris of a planetary system, these cool white dwarfs have featureless optical spectra. Until quite recently, very little was known about the incidence of magnetic fields in these objects. However, when observed with polarimetric techniques, a significant number of featureless white dwarfs reveal strong magnetic fields in their optical continuum spectra. Measuring the occurrence rate and strength of magnetic fields in old white dwarfs may help us to understand how these fields are generated and evolve. We report the results of an ongoing survey of cool white dwarfs with the high-precision broad-band polarimeter DIPOL-UF, which is deployed at the Nordic Optical Telescope on La Palma, Spain. This survey has led to the firm discovery of 13 cool magnetic white dwarfs in the solar neighborhood so far, including six new detections that we report in this paper.

==> Table_Log_STD.tex <==
\begin{table*}
\caption{\label{Tab_Log_Std} Observing log of bright non polarised standard stars, and of the highly polarised MWD WD\,1900$+$705. 
So far, this table incorporate only the values of the non polarised stars measured in the run of November 2023. Civilian dates and
exposure time are still missing.
Polarisation values are given assuming as instrumental polarisation the values of 
$x.xxx \pm y.yyy$\,\%, 
$x.xxx \pm y.yyy$\,\% and 
$z.zzz \pm z.zzz$\,\% 
in the $B'$, $V'$ and $R'$ filters, respectively.}
\begin{center}
\begin{tabular}{lcccrr@{$\pm$}lr@{$\pm$}lr@{$\pm$}l}
\hline\hline
\multicolumn{1}{c}{STAR} & DATE & UT & JD -- & Exp. & \multicolumn{6}{c}{$V/I$ (\%)} \\
                         &yyyy-mm-dd & hh:mm &2400000 &\multicolumn{1}{c}{(s)} &
\multicolumn{2}{c}{$B'$} &\multicolumn{2}{c}{$V'$} &\multicolumn{2}{c}{$R'$} \\
\hline
HD\,19034      & 2024-02-07   &       & 60348.3276&   &$ -0.0001$& 0.0017&$ -0.0003$& 0.0013 &$ -0.0010$&  0.0007 \\
HD\,24206      & 2024-02-03   &       & 60344.3279&   &$  0.0020$& 0.0017&$ -0.0052$& 0.0024 &$ -0.0027$&  0.0023 \\
HD\,28483      & 2024-02-04   &       & 60345.3240&   &$  0.0016$& 0.0013&$ -0.0024$& 0.0012 &$ -0.0005$&  0.0008 \\ 
HD\,31412      & 2024-02-05   &       & 60346.3561&   &$ -0.0001$& 0.0017&$ -0.0007$& 0.0009 &$  0.0017$&  0.0008 \\
HD\,49736      & 2024-02-06   &       & 60347.3262&   &$ -0.0008$& 0.0011&$ -0.0015$& 0.0009 &$  0.0012$&  0.0009 \\
HD\,58781      & 2023-11-17   &       & 60265.7656&   &$  0.0026$& 0.0009&$ -0.0008$& 0.0011 &$  0.0016$&  0.0013 \\
HD\,63814      & 2023-11-18   &       & 60266.7668&   &$ -0.0020$& 0.0010&$ -0.0042$& 0.0007 &$ -0.0013$&  0.0006 \\
HD\,65629      & 2023-11-19   &       & 60267.7625&   &$  0.0039$& 0.0011&$  0.0034$& 0.0013 &$  0.0006$&  0.0008 \\
HD\,207966     & 2023-11-16   &       & 60265.3039&   &$  0.0030$& 0.0014&$ -0.0034$& 0.0009 &$  0.0014$&  0.0009 \\
HD\,215550     & 2023-11-17   &       & 60266.3018&   &$  0.0007$& 0.0008&$ -0.0006$& 0.0006 &$  0.0027$&  0.0008 \\
HD\,224156     & 2023-11-18   &       & 60267.3036&   &$  0.0006$& 0.0011&$ -0.0019$& 0.0011 &$  0.0013$&  0.0010 \\
HD\,202108     & 2023-11-19   &       & 60268.3031&   &$  0.0003$& 0.0015&$ -0.0013$& 0.0009 &$  0.0017$&  0.0008 \\
WD\,1900$+$705 & 2022-11-21 & 19:49 & 59905.326 &   &$  3.759 $& 0.013 &$  3.591 $& 0.031  &$  3.848 $&  0.028  \\  
               & 2023-03-28 & 06:01 & 60031.750 &   &$  3.700 $& 0.015 &$  3.533 $& 0.026  &$  3.810 $&  0.016  \\
               & 2023-11-16 & 20:00 & 60265.333 &   &$  3.709 $& 0.009 &$  3.499 $& 0.016  &$  3.784 $&  0.016  \\     
\hline
\end{tabular}
\end{center}
\end{table*}

